C-Disentanglement: Discovering Causally-Independent Generative Factors under an Inductive Bias of Confounder

Representation learning assumes that real-world data is generated by a few semantically meaningful generative factors (i.e., sources of variation) and aims to discover them in the latent space. These factors are expected to be causally disentangled, meaning that distinct factors are encoded into separate latent variables, and changes in one factor will not affect the values of the others. Compared to statistical independence, causal disentanglement allows more controllable data generation, improved robustness, and better generalization. However, most existing work assumes unconfoundedness in the discovery process, that there are no common causes to the generative factors and thus obtain only statistical independence. In this paper, we recognize the importance of modeling confounders in discovering causal generative factors. Unfortunately, such factors are not identifiable without proper inductive bias. We fill the gap by introducing a framework entitled Confounded-Disentanglement (C-Disentanglement), the first framework that explicitly introduces the inductive bias of confounder via labels from domain expertise. In addition, we accordingly propose an approach to sufficiently identify the causally disentangled factors under any inductive bias of the confounder. We conduct extensive experiments on both synthetic and real-world datasets. Our method demonstrates competitive results compared to various SOTA baselines in obtaining causally disentangled features and downstream tasks under domain shifts.

==> sections/appendices/app_2_derive_eval.tex <==
\section{Related Work}
\label{app:related-work}

\noindent\textbf{Disentangled Representations}
The pursuit for disentangled representation can be dated to the surge of representation learning and is always closely associated with the generative process in modern machine learning, following the intuition that each dimension should encode different features. 
\cite{chen2016infogan} attempts to control the underlying factors by maximizing the mutual information between the images and the latent representations. \cite{eastwood2018framework} propose a quantitative metric with the information theory. They evaluate the disentanglement, completeness, and informativeness by fitting linear models and measuring the deviation from the ideal mapping. \cite{higgins2016beta, kim2018disentangling, chen2018isolating, mathieu2019disentangling} encourage statistical independence by penalizing the Kullback-Leibler divergence (KL) term in the VAE objective. However, the non-causal definitions of disentanglement fail to consider the cases where correlated features in the observational dataset can be disentangled in the generative process. Such a challenge is well-approached through a line of research from the causal perspective.

\noindent\textbf{Causal Generative Process.}
Causal methods are widely used for eliminating spurious features in various domains and improving understandable modelling behaviours\cite{wang2020causal, xu2022patchmix, liu2023cat}. It is not until \cite{suter2019robustly} that it was introduced for a strict characterization of the generative process.
\cite{suter2019robustly} first provided a rigorous definition of a causal generative process and the definition of disentangled causal representation as the non-existence of causal relationships between two variables, i.e., the intervention on one variable does not alter the distribution of the others. The authors further introduce \textit{interventional robustness} as an evaluation metric and show its advantage on multiple benchmarks. \cite{reddy2022causally} follow the path of \cite{suter2019robustly} and further propose two evaluation metrics and the Candle dataset. The confounded assumption allows for correlation in the latent space without tempering with the disentanglement in the data generative. Despite effective evaluation tools, there is still a missing piece on how to infer a set of causally disentangled features. Using the proposed evaluation metric as regulation, the model implicitly assumes unconfoundedness and it falls back to finding statistical independence in the latent space. The problem of unrealistic unconfoundedness assumption is identified by \cite{wang2021desiderata}. They assume that confounders exist but they are unobservable. They further propose an evaluation metric considering the existence of confounders, that causally disentangled latent variables have independent support measured by the IOSS score. Similar to the evaluation metrics introduced in \cite{suter2019robustly, reddy2022causally}, IOSS is also a necessary condition of the causal disentanglement. More importantly, as in previous work focusing on obtaining statistical independence, such a regulation suffers from the identifiability issue. 

\noindent\textbf{Weak Supervision for Inductive Bias.}
The identifiability issue in unsupervised disentangled representation learning is first identified in \cite{locatello2019challenging}. Specifically, they show from the theory that such a learning task is impossible without inductive biases on both the models and the data.  Naturally, a series of weak-supervised or semi-supervised methods~\cite{chen2020weakly, ahuja2022weakly, brehmer2022weakly} are proposed with a learning objective of statistical independence or alignment.  In this paper, we take a step further for the confounding assumption, assuming that the confounders are observable with proper inductive bias so that the latent representation can be better identified.
We, similarly, adopt partial labels of the dataset as the supervision signal. We treat the labels as a source of possible confounders and allow the learning of correlated but causally disentangled latent generative factors to be learned.  
 







==> sections/appendices/app_rebuttal_tables.tex <==
\clearpage

\section{Additional Results for Rebuttal}

\textbf{To Reviewer Mytf}

\input{tex/tables/rebuttals/added_UC}

\textbf{To Reviewer TdLu and Reviewer Mytf}

\input{tex/tables/rebuttals/random_label_celebA}




\textbf{To Reviewer j8n4}

\input{tex/tables/rebuttals/added_baselines}


\textbf{Reference}:

[1]Rombach, Robin, et al. "High-resolution image synthesis with latent diffusion models." Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. 2022.

[2]Jeon, Insu, et al. "Ib-gan: Disentangled representation learning with information bottleneck generative adversarial networks." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 35. No. 9. 2021


==> sections/motivations.tex <==
The commonly assumed notion of disentanglement is quite restrictive for complex models where the true generative factors are not independent, very large in number, or where it cannot be reasonably assumed that there is a well-defined set of “true” generative factors (as will be the case for many, if not most, real datasets). 

Problem settings:

Our settings are that we are given a dataset, and a set of partial labels, or potential generating factors. we would like to induce a set of causally independent features. 

==> tex/plots/dag.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-1.5em}
% \centering
% \begin{framed}
%     \includegraphics[width=\textwidth]{figures/causal_dag.pdf} 
% \end{framed}
% \caption{To be filled}
% \vspace{-1em}
% \label{fig:dag}
% \end{wrapfigure}

\begin{figure*}[!htbp]
\begin{center}
    \begin{subfigure}[t]{0.31\textwidth}
    \includegraphics[width=\textwidth]{figures/dag1.pdf}
    \caption{plot 1}
    \label{subfig:no-causal}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
    \includegraphics[width=\textwidth]{figures/dag2.pdf}
    \caption{plot 2} 
    \label{subfig:single-cause}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
    \includegraphics[width=\textwidth]{figures/dag3.pdf}
    \caption{plot 3} 
    \label{subfig:common-cause}
    \end{subfigure}
    \end{center}

\caption{to be filled}
\label{fig:causal-dag}
\vspace{-0.5em}
\end{figure*}

==> tex/plots/encoder_decoder.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.2\textwidth]{figures/encoder_decoder.pdf}
    \caption{Caption}
    \label{fig:coufounded-causal-process}
\end{figure}

==> tex/plots/ground_truth.tex <==
\begin{wrapfigure}{r}{0.39\textwidth}
\vspace{-.5em}
\centering
    \includegraphics[width=.39\textwidth]{figures/ground_truth.pdf} 
\caption{Ground truth generative process of a fruit dataset.}
\label{fig:ground-truth}
\vspace{-1em}
\end{wrapfigure}

==> tex/plots/ood.tex <==
% \begin{wrapfigure}{r}{0.6\textwidth}
% \vspace{-1.5em}
% \centering

%     \includegraphics[width=.6\textwidth]{figures/ood.png} 

%  \caption{\textbf{Classification under distribution shift.} We compare \model with $\beta$-VAE and Causal-Rep under different levels of distribution shifts from the source domain (object hue correlates to object shape) to the target domain (no correlation between object hue and shape) on a synthetic 3dshape dataset. We report the classification accuracy on the target distribution (T) and the performance gap between the source distribution and the target distribution (S-T).}
% \vspace{-1em}
% \label{fig:ood}
% \end{wrapfigure}

==> tex/tables/compare_with_ground_truth.tex <==
\begin{table}[!htbp]
\caption{\textbf{Compare learned feature with ground truth generative factors on 3d shape dataset.} }
  \label{tab:reconstruction-candle}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lcc}
    \toprule                 
    \textbf{Methods} & \textbf{MIC} & \textbf{TIC} \\
    \midrule
    \multicolumn{1}{l}{VAE}          &  & \\
    \multicolumn{1}{l}{$\beta$-VAE}  &  & \\
    \multicolumn{1}{l}{FactorVAE}    & & \\
    \midrule
    \multicolumn{1}{l}{CAUSAL-REP}   && \\
    \midrule
    \multicolumn{1}{l}{cVAE}         & & \\
    \multicolumn{1}{l}{GMVAE}        & & \\
    \midrule
    \multicolumn{1}{l}{\model} & & \\
  \bottomrule
\end{tabular}
}
\end{table}

==> tex/tables/rebuttals/added_UC.tex <==
\begin{table}[!htbp]
\renewcommand\thetable{1} 
\caption{\textbf{UC score (the higher, the better) on CelebA.} We use annotation attributes as a proxy of the ground truth generative factors (here we use label eyeglasses, smiling and wearing hat as generative factors and compute UC score accordingly. }
  \label{tab:added-baselines}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lccccccc}
    \toprule                 
    \textbf{UC}$\uparrow$ & \textbf{ours} & VAE & $\beta$-VAE & FactorVAE  & CAUSAL-REP &  cVAE  & GMVAE \\
    \midrule
      - &  \textbf{0.24}   & 0.09  & 0.09    & 0.08  & 0.16 & 0.11 & 0.08 \\
  \bottomrule
\end{tabular}
}
\end{table}



==> tex/tables/rebuttals/added_baselines.tex <==
\begin{table}[!htbp]
\renewcommand\thetable{3} 
\caption{We provide two baseline results on Latent Diffusion and IB-GAN. }
  \label{tab:added-baselines}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lccccccc}
    \toprule                 
    \textbf{Methods} & \textbf{IOSS} $\downarrow$  & \textbf{D} $\uparrow$  & \textbf{UC} $\uparrow$ & \textbf{CG} $\uparrow$ &  \textbf{MIC} $\uparrow$ & \textbf{TIC} $\uparrow$ & \textbf{IRS} $\uparrow$\\
    \midrule
    \multicolumn{1}{l}{Latent Diffusion [1]}  & 0.67 & 0.15 &  0.17   & 0.19 & 19.7 &  16.1 & 0.52\\
    \multicolumn{1}{l}{IB-GAN [2]}  & 0.61 & \textbf{0.18} &  0.21     & 0.31 & 21.8 & 17.4 & 0.74\\
    \multicolumn{1}{l}{ours}   &  \textbf{0.34} & 0.16 &   \textbf{0.32}    & \textbf{0.41}  & \textbf{31.9} & \textbf{20.2} & \textbf{0.89} \\
  \bottomrule
\end{tabular}
}
\end{table}

==> tex/tables/rebuttals/random_label_celebA.tex <==
\begin{table}[!htbp]
\renewcommand\thetable{2} 
\caption{\textbf{Compare with baselines in image generation task on celebA.} We provide additional information on how randomly selected $C$ affect the model performance on real-world celebA dataset. We report the averaged result of 10 runs.}
  \label{tab:reconstruction-candle-celebA}
  \begin{center}
  \resizebox{.7\textwidth}{!}{ \small
  \begin{tabular}{lccc}
    \toprule           
    \textbf{Methods} & \textbf{Recon} $\downarrow$ & D $\uparrow$ & \textbf{IOSS} $\downarrow$\\
    \midrule
    \multicolumn{1}{l}{VAE}          & 0.33       &  0.11 &  0.78   \\
    \multicolumn{1}{l}{$\beta$-VAE}  & 0.27       &  0.15 &  0.74  \\
    \multicolumn{1}{l}{FactorVAE}    & 0.25       &  \textbf{0.17} &  0.68  \\
    \midrule
    \multicolumn{1}{l}{CAUSAL-REP}   & 0.29       &  0.16 &  0.34  \\
    \midrule
    \multicolumn{1}{l}{cVAE}         & 0.32      & 0.14  & 0.64  \\
    \multicolumn{1}{l}{GMVAE}        & 0.30      &  0.13 & 0.71  \\
    \midrule
    \multicolumn{1}{l}{\method (ours)} & \textbf{0.18} &  0.12 & \textbf{0.21} \\
    \multicolumn{1}{l}{\method-rand-avg (ours)} & 0.19${\small \pm 0.014}$ &  0.14${\small \pm 0.019}$ & 0.22${\small \pm 0.005}$ \\
  \bottomrule
\end{tabular}
}
\end{center}
\end{table}
